DeepSeq: Deep Sequential Circuit Learning

Circuit representation learning is a promising research direction in the electronic design automation (EDA) field. With sufficient data for pre-training, the learned general yet effective representation can help to solve multiple downstream EDA tasks by fine-tuning it on a small set of task-related data. However, existing solutions only target combinational circuits, significantly limiting their applications. In this work, we propose DeepSeq, a novel representation learning framework for sequential netlists. Specifically, we introduce a dedicated graph neural network (GNN) with a customized propagation scheme to exploit the temporal correlations between gates in sequential circuits. To ensure effective learning, we propose to use a multi-task training objective with two sets of strongly related supervision: logic probability and transition probability at each node. A novel dual attention aggregation mechanism is introduced to facilitate learning both tasks efficiently. Experimental results on various benchmark circuits show that DeepSeq outperforms other GNN models for sequential circuit learning. We evaluate the generalization capability of DeepSeq on a downstream power estimation task. After fine-tuning, DeepSeq can accurately estimate power across various circuits under different workloads.

==> downstream_task-bak.tex <==
\section{Downstream Tasks}\label{task}
% \usepackage{tabularray}
\begin{table}
\centering
\caption{The Statistics of Test Data}
\label{TAB:TestData}
\begin{tabular}{@{}llllll@{}}
\toprule
Design   Name & Description               & \# Nodes \\ \midrule
noc\_router   & Network-on-Chip router    & 5,246    \\
pll           & Phase locked loop         & 18,208   \\
ptc           & PWM/Timer/Counter IP core & 2,024    \\
rtcclock      & Real-time clock core      & 4,720    \\
ac97\_ctrl    & Audio Codec 97 controller & 14,004   \\
mem\_ctrl     & Memory controller         & 10,733   \\ \bottomrule
\end{tabular}
\end{table}
In this section, we evaluate the performance of DeepSeq on two downstreams tasks: \emph{Power Estimation} and \emph{Reliability Analysis}. These tasks can be formulated as a function of underlying circuit structure and logic information, therefore, they help use to evaluate DeepSeq in a fair manner. To prepare the test data, we select six sequential circuits from Opencore~\cite{takeda2008opencore} that are about $1 - 2$ order-of-magnitude larger than the ones used during pre-training. The descriptions of these circuits are listed in Tab.~\ref{TAB:TestData}.
\label{sec:power}
\subsection{Evaluation on Power Estimation}
After designing a general model for sequential circuit learning, we apply it on a downstream \textit{dynamic power estimation task}~\cite{tsui1995power}. Specifically, we describe the performance of DeepSeq on netlist-level power estimation. %Since power consumption is estimated by analyzing the circuit switching activity (transition probability), it makes DeepSeq a suitable model for this task. 
Formally, the circuit dynamic power is characterized as $P = \frac{1}{2} C V_{dd}^2 y_{avg}^{TR}$, wherein $C$ is the capacitance, $V_{dd}$ is the supply voltage, and $y_{avg}^{TR}$ is the average transition probability of all gates. 

The existing power estimation methods mainly fall into two categories: simulative and non-simulative. The simulative methods~\cite{kang1986accurate} rely on the simulation of a huge number of sequential patterns to calculate the switching activities. Although such simulation-based power estimation is accurate, %and considered as the ground-truth power consumption in a specific workload, 
it is not practical for modern large-scale circuit designs due to their unacceptable runtime~\cite{kang1986accurate}. The non-simulative methods~\cite{kapoor1994improving, ghosh1992estimation} %burch1988pattern, } 
are pattern-free %and estimate the inherent switching activity under random patterns. Most non-simulative methods
and use some heuristics or hand-crafted rules to estimate the power in a polynomial %or even linear 
time. However, they produce inaccurate results on structures such as reconvergence fanouts and cyclic FFs~\cite{kapoor1994improving}. 

%\subsubsection{Fine-tuning of DeepSeq for Power Estimation}
\subsubsection{Out-of-Distribution Transition Probabilities of Large Circuits}\label{Sec:power:finetuning}
\iffalse
We observe that transition probabilities follow an uneven distribution, thus causing an imbalanced regression problem. Since power estimation mainly relies on transition probabilities prediction, therefore, we address this issue by replacing the L1 loss with shrinkage loss~\cite{lu2018deep}. As shrinkage loss is specifically proposed to deal with the imbalance regression problem, it helps to further enhance the DeepSeq performance.  % We observe that DeepSeq trained with shrinkage loss performs better mprove the performance of DeepSeq.  out that the performance of DeepSeq
%two different loss functions i.e., focal loss and shrinkage loss, proposed to deal with the imbalance regression problem and compare their performance with the DeepSeq trained with L1 loss function. Table~\ref{Tab:Loss} shows the result. Among all settings, DeepSeq with shrinkage loss performs best. Since focal loss penalizes both easy and hard examples, it has caused a negative impact on DeepSeq's performance. 
%After analyzing the results from Table~\ref{TAB:Comparison} and Table~\ref{Tab:Loss},%we select DeepSeq trained with Shrinkage Loss as our final proposed model. 
\fi

We apply the pre-trained DeepSeq model for the power estimation on real sequential circuits that are substantially larger and different from our pre-training dataset. The accuracy of power estimation is subject to two factors, i.e., circuit structure and the impact of a workload on circuit gates and FFs. The pre-trained DeepSeq has already encoded the structural information and computational behavior of sequential circuits. We observe that the impact of random workloads (distribution of transition probabilities) on these large circuits are quite different than on the small circuits used for pre-training. Particularly, when we simulate a workload, it only activates a few modules in the real applications. 
According to our empirical results, a large part (around $70\%$ of total gates) in these large circuits show no transition activities under a random workload due to low power design~\cite{kathuria2011review}. 

Therefore, to learn the impact of workloads on large circuits (new distribution of transition probabilities) and accurately infer the power, we fine-tune DeepSeq on these large practical circuit designs. The fine-tuning dataset is generated with the same pipeline as Sec.~\ref{Model}. Our empirical study shows that, after fine-tuning with $1,000$ different workloads on a circuit, DeepSeq can generalize to arbitrary workloads for that circuit.

\iffalse
\textcolor{red}{Correct the arguments. 1. Structural \& computational information, outperform baseline model,
We want to apply on PE, depends TR, Workload behavior on large is different than training data (section component active), fine-tuning large circuit with 1k workloads, DeepSeq is generalizable to infinite workloads} 


Although DeepSeq model learns a better representation for sequential netlists than the baseline model on the training dataset (shown in Sec.~\ref{Sec:Exp:Dataset}), the accuracy of predicted transition probability on the real large circuits is still not enough. Before applying DeepSeq to estimate power consumption, we fine-tune the pre-trained model to learn the switching activities with a signal circuit. The fine-tuning dataset contains $1$ circuits with $1,000$ different random workloads, which are generated with the same pipeline as Sec.~\ref{Model}. 
\fi

\subsubsection{Experimental Settings}
%In this experiment, we select six sequential circuits from Opencore~\cite{takeda2008opencore} that are about $1 - 2$ order-of-magnitude larger than the ones used during pre-training. The descriptions of these circuits are listed in Tab.~\ref{TAB:TestPE}.
We select a non-simulative power estimation method~\cite{ghosh1992estimation} and a learning based netlist-level power estimation method, i.e., Grannite~\cite{zhang2020grannite} as the baselines for comparison. Nevertheless, there are more learning based power estimations methods~\cite{zhou2019primal,lin2022powergear}. But they either estimate power at RTL level~\cite{zhou2019primal} or for FPGA HLS~\cite{lin2022powergear}. On the contrary, DeepSeq targets netlist-level power estimation. Therefore, we omit the comparison with these methods. 

We implement Grannite in a unified framework with DeepSeq using PyTorch Geometric (PyG)~\cite{pyg} package. To enable a fair comparison, we keep the same training data for Grannite that we use for Deeseq training, (see Tab.~\ref{TAB:TrainData} and Sec.~\ref{Sec:Exp:Dataset} for more details). However, we generate new node and edge features of training circuits, according to the settings proposed in Grannite. After that, similar to DeepSeq, we train Grannite for 50 epochs using L1 loss. To be noted, Grannite predicts the transition probabilities only for combinational logic in sequential netlist, whereas DeepSeq predicts the transition probabilities for all components in sequential netlists, i.e., PIs, logic gates, FF.

As describe in Sec.~\ref{Sec:power:finetuning}, the distribution of transition probabilites on large circuit designs are quite different than the distribution on training dataset that consists of small circuits. Therefore, similar to DeepSeq, we fine-tune Grannite on these large practical circuit designs. On the one-hand, it ensures a fair comparison with DeepSeq. On the other-hand, it is consistent with training strategy proposed in Grannite, i.e., they train and infer results on real large circuits.

%to learn the impact of workloads on larger circuits (new distribution of transition probabilities) and accurately infer the power, we fine- tune DeepSeq on these large practical circuit designs. 



%During inference, we parse the testbench file of test circuits(see Tab.~\ref{TAB:TestData})During inference, % which serves as the workload information to DeepSeq model and the baseline methods as workload. 
In practice, power estimation is performed on circuits with multiple gate types.
However, our model only supports input circuits in AIG format. Therefore during inference, to apply our model on test data (large circuits with multiple gate types) for power estimation, we decompose each gate into a combination of AND gates and NOT gates without any optimization. The fanout gate in the resulting combination has the same switching activity as the original node. Note that, we only record probabilities of the fanout gates in all converted combinations. To generate the workload of our test circuits, we parse their corresponding testbench files and collect the transition probability and logic probability of each PI. The collected information defines the workloads of underlying circuits. 

The power estimation pipeline is illustrated in Fig.~\ref{FIG:power}. We set the transition probability achieved by the logic simulation as the ground truth (GT). The probabilistic baseline method~\cite{ghosh1992estimation} provides the approximated transition probability based on a non-simulative method. In comparison, learning based baseline method, i.e., fine-tuned Grannite % and DeepSeq 
predicts the gate-level transition probabilities. As mentioned before, Grannite only predicts the transition probabilities of combinational logic whereas DeepSeq predicts the transition probabilities of all components in sequential netlists, i.e., PIs, logic gates, FF. Therefore, for Grannite based power estimation, we follow their settings and use RTL level simulation results to obtain transition probabilities of PIs and FFs. %, we use the GT transition probabilites.  
 This helps us to infer the complete sequential netlist-level power. % and enables comparison with DeepSeq. 
For DeepSeq based power estimation, we run the following two settings: 
\vspace{2pt}
\begin{enumerate}
    \item We use DeepSeq to infer transition probabilities of combinational logic only and use RTL level simulation to get transition probabilities of PIs and FFs. This setting is consistent with the settings in Grannite experiment and enables a fair comparison. We named it as \emph{DeepSeq-Combinational}.
    \vspace{2pt}
    \item We use DeepSeq to infer transition probabilities for complete sequential netlist. This settings is consistent with DeepSeq objective. The results under this setting shows the DeepSeq capacity to correctly encode the complete sequential circuit behavior.
    %shows the pthe DeepSeq 
    %Since DeepSeq is focus to learn the sequential circuit behavior. combinational logic only and use RTL level simulation to get transition probabilities for PIs and FFs. This setting is consistent with grannite settings and enables a fair comparison.
\end{enumerate}
\vspace{2pt}

%we use the GT transition probabilities for PIs and FFs in Grannite.
The resulting transition probabilities from all these methods are translated into four Switching Activity Interchange Format (SAIF) files. After that, we input these files into a commercial power analysis tool that computes the average power with a TSMC 90nm standard cell library. Finally, we can get the ground-truth power consumption (GT Power), non-simulated baseline power (Probabilistic Power), learning based baseline power (Grannite Power), DeepSeq-Combinational estimation power (DeepSeq-Comb. Power), and DeepSeq estimated power (DeepSeq Power). 

\begin{figure}[t!]
    \vspace{-10pt}
	\centering
	\includegraphics[width=0.9\linewidth]{fig/power_pipeline.pdf}
	\vspace{-5pt}
	\caption{The pipeline of power estimation}
	\label{FIG:power}
	\vspace{-10pt}
\end{figure}
% \usepackage{tabularray}

\iffalse
\begin{table*}[!t]
\vspace{-10pt}
\centering
\caption{The Results of Power Estimation on 11 Large Real Circuits} \label{TAB:TestPE}
\begin{tabular}{@{}llllll|ll@{}}
\toprule
Design   Name & Description               & \multicolumn{1}{l|}{\# Nodes}  & \multicolumn{1}{l|}{GT (mW)}   & Baseline (mW) & Error            & DeepSeq (mW) & Error           \\ \midrule
noc\_router   & Network-on-Chip router    & \multicolumn{1}{l|}{5,246}     & \multicolumn{1}{l|}{0.653}     & 0.696         & 6.58\%           & 0.643        & 1.52\%          \\
pll           & Phase locked loop         & \multicolumn{1}{l|}{18,208}    & \multicolumn{1}{l|}{0.936}     & 1.115         & 19.12\%          & 0.960        & 2.51\%          \\
ptc           & PWM/Timer/Counter IP core & \multicolumn{1}{l|}{2,024}     & \multicolumn{1}{l|}{0.247}     & 0.184         & 25.55\%          & 0.239        & 3.20\%          \\
rtcclock      & Real-time clock core      & \multicolumn{1}{l|}{4,720}     & \multicolumn{1}{l|}{0.463}     & 0.522         & 12.84\%          & 0.442        & 4.43\%          \\
ac97\_ctrl    & Audio Codec 97 controller & \multicolumn{1}{l|}{14,004}    & \multicolumn{1}{l|}{3.353}     & 2.474         & 26.22\%          & 3.261        & 2.74\%          \\
mem\_ctrl     & Memory controller         & \multicolumn{1}{l|}{10,733}    & \multicolumn{1}{l|}{1.365}     & 1.471         & 7.77\%           & 1.303        & 4.54\%          \\ \midrule
\textbf{Avg.} & \textbf{}                 & \textbf{} & \textbf{} & \textbf{}     & \textbf{16.35\%} & \textbf{}    & \textbf{3.16\%} \\ \bottomrule
\end{tabular}
\vspace{-10pt}
\end{table*}
\fi
% \usepackage{tabularray}
% \usepackage{tabularray}

\iffalse
\begin{table*}[!t]
\centering
\caption{The Results of Power Estimation on 6 Large-Scale Circuits} \label{TAB:TestPE}
\begin{tabular}{@{}ll|ll|ll|ll@{}}
\toprule
Design   Name & {GT (mW)} & Probabilistic (mW) & Error.           & Grannite (mW) & Error.           & DeepSeq (mW) & Error.          \\ \midrule
noc\_router   & {0.653}   & 0.696              & 6.58\%           & 0.641         & 1.85\%          & 0.643        & 1.53\%          \\
pll           & {0.936}   & 1.115              & 19.12\%          & 0.829         & 11.41\%         & 0.960        & 2.56\%          \\
ptc           & {0.247}   & 0.184              & 25.55\%          & 0.222         & 10.20\%         & 0.239        & 3.24\%          \\
rtcclock      & {0.463}   & 0.522              & 12.84\%          & 0.437         & 5.72\%          & 0.442        & 4.54\%          \\
ac97\_ctrl    & {3.353}   & 2.474              & 26.22\%          & 3.943         & 17.60\%         & 3.261        & 2.74\%          \\
mem\_ctrl     & {1.365}   & 1.471              & 7.77\%           & 1.309         & 4.10\%          & 1.303        & 4.54\%          \\ \midrule
\textbf{Avg.} &                              &                    & \textbf{16.35\%} &               & \textbf{8.48\%} &              & \textbf{3.19\%} \\ \bottomrule
\end{tabular}
\end{table*}
\fi


\begin{table*}[!t]
\centering
\caption{The Results of Power Estimation on 6 Large-Scale Circuits} \label{TAB:TestPE}
\begin{tabular}{@{}ll|ll|ll|ll@{}}
\toprule
Design   Name & {GT (mW)} & Probabilistic (mW) & Error           & Grannite (mW) & Error          & DeepSeq (mW) & Error         \\ \midrule
noc\_router   & {0.653}   & 0.696              & 6.58\%           & 0.641         & 1.85\%          & 0.643        & 1.53\%       \\
pll           & {0.936}   & 1.115              & 19.12\%          & 0.829         & 11.41\%         & 0.960        & 2.56\%       \\
ptc           & {0.247}   & 0.184              & 25.55\%          & 0.222         & 10.20\%         & 0.239        & 3.24\%   \\
rtcclock      & {0.463}   & 0.522              & 12.84\%          & 0.437         & 5.72\%          & 0.442        & 4.54\%         \\
ac97\_ctrl    & {3.353}   & 2.474              & 26.22\%          & 3.943         & 17.60\%         & 3.261        & 2.74\%          \\
mem\_ctrl     & {1.365}   & 1.471              & 7.77\%           & 1.309         & 4.10\%          & 1.303        & 4.54\%       \\ \midrule
\textbf{Avg.} &                              &                    & \textbf{16.35\%} &               & \textbf{8.48\%} &              & \textbf{3.19\%}   \\ \bottomrule
\end{tabular}
\end{table*}




\begin{table*}[!t]
\centering
\caption{The Results of Power Estimation on ac97\_ctrl with Different Workloads} \label{TAB:PEac97}
\begin{tabular}{@{}ll|ll|ll|ll@{}}
\toprule
Workload ID   & {GT (mW)} & Probabilistic (mW) & Error.           & Grannite (mW) & Error.           & DeepSeq (mW) & Error.          \\ \midrule
W0            & {3.353} & 2.474     & 26.22\%          & 3.943    & 17.60\%          & 3.261     & 2.74\%         \\
W1            & {3.349} & 3.082     & 7.97\%           & 3.581    & 6.93\%          & 3.219     & 3.88\%          \\
W2            & {2.758} & 2.269     & 17.73\%          & 2.826    & 2.47\%          & 2.697     & 2.21\%          \\
W3            & {3.414} & 2.965     & 13.15\%          & 3.640    & 6.62\%          & 3.322     & 2.69\%          \\
W4            & {6.696} & 5.860     & 12.49\%          & 6.930    & 3.49\%          & 6.607     & 1.33\%          \\ \midrule
\textbf{Avg.} & \textbf{}                  & \textbf{} & \textbf{15.51\%} &          & \textbf{7.42\%} & \textbf{} & \textbf{2.57\%} \\ \bottomrule
\end{tabular}
%\vspace{-10pt}
\end{table*}
\vspace{5pt}

\begin{table}[]
\centering
\caption{The Results of Reliability Analysis on 6 Large Scale} \label{TAB:Relia}
\begin{tabular}{@{}ll|ll|ll@{}}
\toprule
Design Name   & GT    & Probabilistic & Error.          & DeepSeq & Error.          \\ \midrule
noc\_router   & 0.9876 & 0.9607        & 2.72\%          & 0.9814  & 0.63\%          \\
pll           & 0.9792 & 0.9501        & 3.95\%          & 0.9857  & 0.35\%          \\
ptc           & 0.9970 & 0.9656        & 3.15\%          & 0.9928  & 0.42\%          \\
rtcclock      & 0.9985 & 0.9812        & 1.73\%          & 0.9969  & 0.16\%          \\
ac97\_ctrl    & 0.9953 & 0.9704        & 2.50\%          & 0.9943  & 0.10\%          \\
mem\_ctrl     & 0.9958 & 0.9767        & 1.92\%          & 0.9936  & 0.22\%          \\ \midrule
\textbf{Avg.} &       &               & \textbf{2.66\%} &         & \textbf{0.31\%} \\ \bottomrule
\end{tabular}
\end{table}
\subsubsection{Results}
%We collect $6$ open-source circuits as testing circuits. The description of these circuits are listed in Tab.~\ref{TAB:TestPE}. As our model only support AIG as input, we covert the netlist into AIG without any optimization before model inference. . 

\paragraph{Power Estimation on the large-scale circuits}
Table~\ref{TAB:TestPE} shows the accuracy achieved by DeepSeq over the baseline methods, where the estimated power based on transition probabilities computed from ground-truth, non-simulated method, Grannite, DeepSeq-Combinational and DeepSeq are abbreviated as GT, Probabilistic, Grannite, DeepSeq-Comb., and DeepSeq, respectively. The results show that the power estimation based on  DeepSeq  model has smaller error than the both baseline methods. Take the circuit \textit{pll} as an example, DeepSeq estimates the power consumption only with $2.56\%$ error, while the probabilistic method and Grannite has $19.12\%$ and $11.41\%$ error, respectively. %Since, in DeepSeq-Comb. setting, the transition probabilities of PIs and FFs are obtained from RTL level simulations,
In DeepSeq-Comb. setting, the error on this circuit further reduces to $2.03\%$, which clearly demostrates the efficacy of DeepSeq over Grannite. 
%to encode the combinational logic and sequential
%Among all test circuits, only on one circuit, i.e., \textit{mem\_ctrl}, Grannite produces smaller power estimation error than DeepSeq. However, the difference between the errors from Grannite and DeepSeq minor, i.e., $0.44\%$. Since, in Grannite based power estimation, the transition probabilities of PIs and FFs comes from GT, we argue that this leads to a slightly better performance of Grannite on \textit{mem\_ctrl} over DeepSeq.
Overall, the probabilistic power estimation method achieves $16.35\%$ error on average and Grannite produces $8.48\%$ error on average whereas DeepSeq show $3.19\%$ error on average, which is much closer to the ground-truth power estimation. %Besides, results from DeepSeq-Comb. further improves the performance by reducing the error to $2.87\%$. 
DeepSeq-Comb. further improves the accuracy by reducing the error to $2.87\%$. %This demonstrates that DeepSeq 
However, the better performance of DeepSeq-Comb. over DeepSeq is evident due to use of RTL level simulations to get the transition probabilites of PIs and FFs in DeepSeq-Comb. setting.  
To conclude, without any dependency on RTL level simulations results, DeepSeq generalizes well to unseen large-scale sequential circuit designs and brings a significant improvement in error reduction, i.e., $80.49\%$ over the probabilistic baseline method and $62.38\%$ over Grannite. % on large-scale circuits.
\textcolor{red}{Improve the above saying}
\vspace{5pt}

\paragraph{Power Estimation with different workloads}
We take the \textit{ac97\_ctrl} as an example to show that DeepSeq is generalizable to a new circuit under many different workloads. We assign $5$ different workloads to this circuit and estimate the power consumption based on the same pipeline as Fig.~\ref{FIG:power}. As illustrated in Tab.~\ref{TAB:PEac97}, DeepSeq achieves only $2.57\%$ error in comparison to GT power estimation, while the probabilistic baseline method and Grannite has $15.51\%$  and $7.42\%$ errors, respectively. We attribute the better performance of DeepSeq to customized propagation scheme and \textit{dual attention} aggregation function. Our results show that DeepSeq is generalizable to unseen large circuits with new workloads and infers effective representation.
\vspace{5pt}

\paragraph{Discussion on Grannite performance in comparison with DeepSeq} 

Table~\ref{TAB:TestPE} clearly demonstrates the superior performance of Grannite and DeepSeq over the probablisitic baseline method for all test circuits. This result is in accordance with the fact that probablisitic methods suffer from inaccurate results at complex circuit structures, e.g., reconvergence fanouts.
In this section, we perform an in-depth comparison between DeepSeq and Grannite, and explain the factors that make DeepSeq perform better than Grannite.
%In this section, we compare the architectural designs of DeepSeq and Grannite in order to gain detailed insights that make DeepSeq perform better than Grannite.

%In this section, we perform the architectural comparison between DeepSeq and Grannite to get detailed insights that leads to better of DeepSeq.$an end-to-end comparison between Grannite and DeepSeq architecture that ex

%In this section, we perform a architectural comparison between DeepSeq and Grannite that leads to better performance of outperforms Grannite. In this section, we closely 
%Therefore, in this section, we compare the performance of Grannite with DeepSeq. %For all test circuits, DeepSeq outperforms Grannite except  \textit{ptc}. However, for \textit{ptc}, the difference between the errors from Grannite and DeepSeq is very small, i.e., 0.44\%.

Power estimation solely relies on the accurate transition probabilities. For sequential netlists, the transition probabilities of all circuit components, i.e., inputs, gates and registers are strongly dependent on the periodic information update. To incorporate this effect, in DeepSeq, we propose a customized propagation scheme (Sect.~\ref{sec:method}). On the contrary, in Grannite, the transition probabilites of circuit's inputs and registers are obtained from RTL simulation and provided as inputs to the model. Given this fixed information, Grannite only processes the combinational logic in a forward pass and learns to infer its transition probabilities. We argue that, in this setting, the periodic information exchange between memory elements and combinational logic is missing. Therefore, the model produces less accurate results.

%'t generalizes well to unseen circuits. 

%for the combinational part of circuit. 

%We argue that, in this setting, the model cannot learn the effect of periodic information update. \textcolor{red}{improve it}.
\iffalse
Besides this, Grannite uses multiple node and edge level features obtained from that truth tables of logics gates, e.g., \textit{intrinsitic transition probability} (node feature) and \textit{pin state to output state correlation} (edge feature). These feature encodes the logic and transition behavior of corresponding gates. Whereas in DeepSeq, gate type is used as the only node feature. Given multiple node and edges level information, it should be easier for Grannite to infer transition probabilities. However, the better performance of DeepSeq proves the capability of its architecture to encode the behavior of sequential netlists. Thanks to the customized propagation scheme and dual attention aggregation function that effectively model the periodic information update in sequential netlists under multi-task learning strategy. %that helps to encode 
%\textcolor{red}{improve it}.
\fi


\subsection{Evaluation on Reliability Analysis}\label{sec:reliability}
To further ensures the generalizability and transferability of pre-trained DeepSeq model, we apply it to another downstream task, i.e., netlist level reliability analysis~\cite{mahdavi2009scrap}. The reliability of a logic circuit is a measure of its vulnerability to permanent, intermittent and transient faults. In this work, we focus on evaluating the reliability of logic circuits in presence of intermittent and transient faults. The existing solutions of reliability analysis are also either simulation based or are analytical methods. The simulation based methods are costly in terms of their large run-time whereas analytical methods are fast but less accurate when dealing with signal correlations and reconvergence fanouts in logic circuits.~\cite{Franco2008SignalPF} provides a heuristic based solution named multiplass-SPRA that produces exact results for reconvergence fanouts but its complexity grows exponentially with the number of fanout sources in the circuit, restricting its application to large circuits designs, similar to simulation based solutions.

\subsubsection{Experimental Settings}
We first fine-tune DeepSeq using the dataset describe in Tab.~\ref{TAB:Comparison} for circuit reliability prediction task. To achieve this, we supervise every node with a 2-d vector containing 0$\rightarrow$1 and 1$\rightarrow$0 error probability. 0$\rightarrow$1 error probability at a node represents the flipping probability when the correct output is 0. Similarly, 1$\rightarrow$0 error probability at a node represents the flipping probability when the correct output is 1. To obtain the ground truth, we first generate 1000 sequential patterns (each pattern consists of 100 clock cycles) for fault-free simulation. Then, using the same patterns, we simulate the circuit again using Monte Carlo method with a 0.05\% error rate. We record the responses from both simulations and calculate the error probabilities. 

% Monte Carlo simulation is performed to obtain the ground truth labels, in which we simulate 1000 sequential pattern (every pattern consists of 100 clock cycles) pairs. Each pattern pair consists of one fault-free simulation and one faulty simulation. We set the error rate as 0.05\%.  

In this experiment, we again use the one-hot encoding of gate type as the only node feature. 
%Each circuit is simulated with 1000 pattern pairs using Monte Carlo method in which the \textcolor{red}{@stone help complete this part and add reference for monte carlo method}.
We keep the same hyper-parameter configurations that we use for pre-training of DeepSeq and fine-tune it for 50 epochs using L1 loss. 
Since there is no learning based reliability analysis solution, we choose an analytical method ~\cite{Jahanirad2018EfficientRE} as a baseline for comparison. The test data used during inference in reported in Tab.~\ref{TAB:TestData}.

\subsubsection{Results}

Tab.~\ref{TAB:Relia} shows the accuracy achieved by DeepSeq over the baseline method, where the estimated power based on transition probabilities computed from ground-truth,analytical method, and DeepSeq are abbreviated as GT, Probabilistic, and DeepSeq, respectively. Results show that DeepSeq outperforms the baseline method for all test circuits. Overall the baseline method achieves $2.66\%$ error on average whereas Grannite produces only $0.31\%$ error on average, which is much closer to the ground-truth reliability estimates. DeepSeq brings a major improvement of $88.35\%$ over the baseline method.

==> preliminaries.tex <==
\section{Preliminaries}\label{sec:preliminary}

